Grasp Stability Analysis with Passive Reactions

[...] We argue that the traditional grasp modeling theory assumes a complexity that most robotic hands do not possess and is therefore of limited applicability to the robotic hands commonly used today. We discuss these limitations of the existing grasp modeling literature and set out to develop our own tools for the analysis of passive effects in robotic grasping. We show that problems of this kind are difficult to solve due to the non-convexity of the Maximum Dissipation Principle (MDP), which is part of the Coulomb friction law. We show that for planar grasps the MDP can be decomposed into a number of piecewise convex problems, which can be solved for efficiently. [...] Thus, we present the first polynomial runtime algorithm for the determination of passive stability of planar grasps. For the spacial case we [...] describe a convex relaxation of the Coulomb friction law and a successive hierarchical tightening approach that allows us to find solutions to the exact problem including the maximum dissipation principle. [...] The generality of our grasp model allows us to solve a wide variety of problems such as the computation of optimal actuator commands. This makes our framework a valuable tool for practical manipulation applications. Our work is relevant beyond robotic manipulation as it applies to the stability of any assembly of rigid bodies with frictional contacts, unilateral constraints and externally applied wrenches. Finally, we argue that with the advent of data-driven methods as well as the emergence of a new generation of highly sensorized hands there are opportunities for the application of the traditional grasp modeling theory to fields such as robotic in-hand manipulation through model-free reinforcement learning. We present a method that applies traditional grasp models to maintain quasi-static stability throughout a nominally model-free reinforcement learning task. [...]

==> acknowledgements.tex <==
%ACKNOWLEDGEMENTS page. 
%This page is optional

\clearpage
\begin{center}

\vspace*{5\baselineskip}
\textbf{\large Acknowledgements}
\end{center}


\begin{flushleft}
\hspace{10mm}Insert your acknowledgements text here. This page is optional, you may delete it if not needed. 
\end{flushleft}
\clearpage

%\pagenumbering{gobble}  %remove page number on summary page




==> problem_overview.tex <==
% Move all of this into introduction. Except for the theory section, which
% goes into the related work. Keep the tension between theory and practice.

\chapter{Problem Overview and Contributions}\label{sec:overview}

\section{Motivation}

The analysis of the stability of a grasp is a foundational aspect of
multi-fingered  robotic manipulation. Determining the ability of a grasp to
resist given disturbances, formulated as external wrenches applied to the
grasped object, is equivalent to computing the stability of a multi-body
system with frictional contacts under applied loads. Problems of this kind are
thus pervasive in grasp analysis and may be encountered in many other
scenarios that require simulation of general rigid bodies with frictional
contacts.

In the context of robotic manipulation the following queries are important in
practical use: 

\begin{itemize}
\item \textit{Given a set of commanded torques and an external
disturbance will the system as described above remain quasistatically
stable?} 
\item We can also formulate the inverse query to obtain useful insight
into how to control the hand: \textit{Given an external disturbance, how must
we command the actuators to guarantee the grasp remains stable?}
\end{itemize}

% Here is an example of a feature we believe was missed by the theory

We argue that these queries are foundational to any robotic manipulation task.
In order to illustrate their place in robotic manipulation let us consider the
grasp in Fig.~\ref{fig:package}. Does the grasp remain stable if we apply
either disturbance $\bm{w}_1$ or $\bm{w}_2$ to the grasped object? In order to
resist those disturbances, contact forces must arise that balance them.
Clearly in either case there exist contact forces that satisfy a simple
friction law (illustrated by red friction cones) and balance the disturbance.
In fact, this is a force closure grasp and hence contact forces exist that
could balance arbitrary disturbances. 

In practice, however, this is not a sufficient criterion for grasp stability.
It is clear that contact forces $\bm{c}_2$ and $\bm{c}_4$ will only arise if
we have previously loaded the grasp such that there is sufficient normal force
at contacts 2 and 4 to sustain the friction forces required: an appropriate
preload is required, or the object will slip out. We could, for example apply
actuator torques at the joints such that the hand 'squeezes' the object and
hence provides such a preload.

We can make a similar argument about contact forces that balance disturbance
$\bm{w}_2$, however if we assume that the joints on the robotic hand are
nonbackdrivable (as is the case with most robotic hands in use today) contact
forces $\bm{c}_1$ and $\bm{c}_3$ will arise entirely passively. The
disturbance will push the object against the fingers, which due to the
nonbackdrivability of the joints provide a rigid support. There is no need for
us to apply any torques at the joints as the grasp will be stable regardless.
We call this \textit{passive resistance}.

\begin{figure}[!t]
\centering
\includegraphics[width=0.6\columnwidth]{graphics/grasp_3.png}
\caption{A grasping scenario where a hand establishes multiple
    frictional contacts (numbered 1-4) with a target object. External
    disturbance $\bm{w}_1$ can be
    resisted by contact forces $\bm{c}_2$ and $\bm{c}_4$; $\bm{w}_2$ by
    contact forces $\bm{c}_1$ and $\bm{c}_3$.}\label{fig:package}
\end{figure}

This start contrast in the requirements for stability serves as an example of
why it is paramount to take into account the kinematics of the hand and its
actuation scheme when attempting to answer the stability queries described
above. A grasp model that accounts for all these effects and can answer these
queries must capture the interplay of contact forces, joint torques and
external wrenches. It must be able to accurately predict how joint torques and
external wrenches are transmitted through the object and distributed across
the contacts taking into account the unilaterality of contacts and
nonbackdrivable joints as well as the nonlinear nature of friction laws.

\section{Manipulation: Theory}

Much of the previous work in this field discussed in~\ref{sec:related} focuses
on two perspectives on robotic grasping.

\subsection{Grasp Stability as a rigid body problem}

A grasp can be viewed as a completely passive fixture. The grasp is made up of
rigid bodies that are either fixed in space (like the 'grounded' base of the
robot), free floating (like the grasped object) or connected by a kinematic
chain (such as the manipulator links.) The bodies comprising the kinematic
chains are connected to each other and --- at least indirectly --- the ground
by bilateral constraints such as hinge joints. Contacts between bodies are
unilateral constraints also satisfying a friction law such as Coulomb
friction. All external forces acting on the bodies such as gravity or
actuation wrenches are known. Such an arrangement is deemed stable if it
remains at rest (all accellerations are zero.)

The works described in~\ref{sec:related_mechanics}
and~\ref{sec:related_dynamics} focusing on the analysis of rigid bodies have
produced very natural formulations based on complementarity problems as well
as numerous relaxations in order to improve efficiency. We could, for example,
attempt to use any of the various dynamics solvers the field has produced to
compute contact forces and calculate a single time step. If all accellerations
remain zero, we deem the grasp stable. Unfortunately, this approach will not
give us definite results.

Any algorithm that makes use of relaxations also introduces artifacts as we
are no longer solving the exact problem as outlined above. These artifacts are
acceptable for the purposes of those algorithms: Dynamics simulation that is
fast enough for use in time sensitive applications such as virtual reality or
deep learning. In our application, however, these artifacts mean that we
cannot rely on the simulation to produce exactly zero accellerations even for
grasps that are truly stable.

Thus, we need to focus on the algorithms that solve the exact problem. Perhaps
the best candidate is the formulation as a mixed nonlinear complementarity
problem (mixed NCP) introduced by Trinkle et al.~\cite{TRINKLE97}. In a
previous paper~\cite{PangTrinkle1996} Pang and Trinkle showed that in the case
of systems initially at rest the existence of a solution is guaranteed.
However, they also note a difficulty in using this formulation for stability
analysis: One must show that \textit{every} solution to the complementarity
problem has a zero accelleration.

Generally, when using a complementarity formulation in a dynamics engine only
one solution is required in order to step the simulation forward in time. This
allows the application of solvers such as Lemke's algorithm, which only finds
a single solution --- if one exists. The only algorithms that find all
solutions to general complementarity problems are enumerative in
nature~\cite{murty1988linear} and therefore computationally complex.

To the best knowledge of the author, the work which has comes closest to
answering the question of stability under the above assumtions is the work by
Pang et al.~\cite{ZAMM643}, which makes use of the complementarity formulation
due to Trinkle et al.~\cite{TRINKLE97}. In special cases, in which the
solution is unique, there is no ambiguity due to multiple solutions and the
single solution to the LCP determines stability. A framework that efficiently
determines stability for general grasps under the rigid body assumption has
not yet been found.

\subsection{Grasp Stability as a grasp force synthesis problem}

The second perspective on robotic grasping introduces the assumption that the
contact wrenches of a grasp can be somehow actively controlled. This can be
done directly through commanding appropriate joint torques or more indirectly
through setting compliance parameter such as servo gains. This assumption
allows the analysis of grasp analysis through the equilibrium equations alone,
where the rigid body approach required treatment of the full dynamics
equations. These methods allow us to compute optimal contact forces and the
joint torques necessary to balance them. Thus, for any specific wrench on the
object encountered throughout a task we can compute the specific optimal joint
torques for stability.

In order to use this in practice, however, we have to make a string of
assumptions:

\begin{enumerate}

\item We assume perfect knowledge of the disturbance to the object
that must be balanced at all times;

\item We assume that we can actively control the contact forces at
every contact;

\item We assume that we can actively control the joint torques required
for equilibrium;

\item We assume that we can accurately control the torque
output of the hand actuators.

\end{enumerate}

In the majority of robotic manipulation tasks these assumptions do not hold. 
First, the exact disturbance wrench acting on an object is difficult to
compute --- it requires knowledge of the mass and inertial properties as well
as the exact trajectory of the object. Any additional disturbance cannot be
accounted for unless the fingers are equipped with tactile sensors. Second,
many robotic hands are kinematically deficient and contain links with limited
mobility. This means, for example, that we cannot directly control the
contact force at a contact on the palm of the hand for instance. Forces at
such a contact can only arise passively by transmission of the disturbance on
the grasped object or forces at other contacts through the object.

Third, the kinematics of the hand may not permit explicit control of the
torques at every individual joint. This is the case for the class of
underactuated hands, where joint torques by definition may not be
independently controlled but are determined by the kinematic composition of
the hand. Finally, most robotic hands use highly geared motors, which makes
accurate sensing and control of the torques at the hand joints all but
impossible.

Therefore, in practice it is rarely the case that contact wrenches are
actively controlled in response to disturbances to the grasp. Unfortunately,
this means that force closure is a necessary but by no means a sufficient
condition for the ability of a grasp to resist arbitrary disturbances. It just
indicates the existence of contact forces that satisfy the friction laws and
can balance the applied disturbance but does not guarantee they will arise,
unless we assume that we are actively controlling the contact forces to that
end.

A method to alleviate some of the limitations due to the above assumptions is
to take into account the flexibility of the object and the elements of the
hand. Bicchi~\cite{BICCHI93} made use of the grasp compliance theory developed
by Cutkosky et al.~\cite{CUTKOSKY_COMPLIANCE} in order to overcome the second
of the assumptions listed above. We could make use of the same theory to model
a grasp without any of the other three assumptions by modeling the grasp as an
entirely passive fixture. Assume the grasp is made up of deformable components
such as series-elastic actuators or the contact itself is deformable due to an
elastic skin covering the finger links. These deformable components would
provide us with constitutive equations such that we can solve for
displacements and hence forces given a specific disturbance.

One obvious limitation of this approach is that the stiffness parameters can
be difficult to obtain, particularly for very stiff hands. Another limitation
was pointed out by Prattichizzo et al.~\cite{PRATTICHIZZO97}: When there is
compliance in the grasp the presence of sliding or breaking contacts does not
necessarily mean the grasp is unstable. Only a subset of contacts may be
required for stability. For illustration, consider a force applied to the
object in Fig.~\ref{fig:package} along the positive $x$-axis that pushes the
object to the right. Only contacts 3 and 4 may be required to balance this
disturbance, so even if contacts 1 and 2 break the grasp remains stable.

This causes an issue as the contact wrench at a breaking or sliding contact is
clearly not described by a compliance relation. At a breaking contact a
compliance relation would lead to a negative normal force, which is
impossible. At a sliding contact the contact force would depend on linearly on
the tangential displacement, which may not satisfy the maximum dissipation
principle or even the friction cone constraint. While Prattichizzo et al. find
approximations that work well for their purposes, there is no efficient way to
apply an approach based on grasp compliance to a problem with potentially
breaking or slipping contacts. 

\section{Manipulation: Praxis}

Having discussed the limitations of the grasp force synthesis theory it is
istructive to think about why robotic hands have not evolved in such a way as
to fulfil the assumptions listed above. We discussed why these assumptions are
difficult to satisfy in practice and why attempts to remove those assumptions
introduce their own limitations. Still, it seems to not provide enough reason
for the schism that separates the theory and the hands commonly in use today.
After all, why build hands that are so far removed from the theory that allows
their analysis? In order to answer this question we must revisit a feature
present in most commonly robotic hands that we have already mentioned in the
Motivation section: Passive resistance due to nonbackdrivable joints. 

Nonbackdrivability arises due to the highly geared actuation of most commonly
used hands. Large gearing ratios between the actuators and the joints mean the
fingers are nonbackdrivable thus providing potentially rigid constraints for
the grasped object. Passive resistance allows practitioners to greatly
simplify robotic grasping. We can often apply actuator torques that close the
fingers around the object without necessarily worrying if these will balance
out once contact is made: the fingers jam as the hand squeezes the object, and
the gearboxes between joints and actuators provide additional structural
torques. If the grasp geometry is adequately chosen, the equilibrium joint
torques arise passively when the fingers squeeze the object between them and a
stable grasp arises. For example, in the grasp in Fig.~\ref{fig:package} it is
sufficient to actively load the joints of one finger. The nonbackdrivability
of the other finger means the object will be stably grasped and equilibrium
joint torques arise passively in the non-actuated finger.

The same phenomenon can allow a grasp to withstand a range of disturbances
applied to the object without a change in the actuator commands. If chosen
wisely, the initially applied preload is sufficient to balance the object
throughout the task and various corresponding different disturbances. This is
the true power of passive resistance.

We believe this characteristic to be the reason why robotic hands without
explicit real-time actuation have become so commonplace. Reactions to
disturbances arising passively due to non-backdrivable actuators remove the
need for complex hand control schemes and the high fidelity sensing they
require. If the grasp geometry and commanded torques are chosen wisely the
grasp will be passively stable to a range of disturbances greatly simplifying
the control of the hand. We simply need to pick a constant command appropriate
to the task. 

So the answer to the question as to why most robotic hands lack the complexity
required for the application of the grasp theory is that practitioners can
rely on passive stability instead. This allows them to form stable grasps,
even though they lack the tools required to analyze them.

On a final note, there is another class of hands commonly found in research
labs today: Underactuated hands. These hands make use of their passive
compliance in order to conform around objects. Soft robotic hands take this
approach to the extreme. All these hands have in common that their passive
behavior greatly simplifies control, which explains their popularity.

\section{Implications for learning in-hand manipulation}

With the more recent drive towards more dexterous manipulation by the deep
learning communitiy, there is renewed demand for highly sensorized hands and
we believe the rich grasping theory that has mostly been forgotten by the
manipulation community is once again becoming relevant.

\section{Contributions}

Our main contributions are two-fold. Firstly, we provide 






The works discussed above are clearly related in spirit to our endeavour.
However, the algorithms developed are either exceedingly computationally
complex or do not take into account all of the effects that characterize
grasps with robotic hands commonly in use. In the following we will develop
computationally efficient algorithms for the analysis of problems as described
in this section

We introduce a quasi-static model that addresses all the constraints above for
general, three-dimensional grasps. We show that inclusion of
the MDP is vital to the physical accuracy and usefulness of such a model and
present a convex relaxation that allows for efficient solution of problems
involving the MDP. While our model is based on a linear approximation of
friction cones, we introduce a computationally efficient method that can
successively tighten this approximation up to the desired accuracy.
A very useful property of tightening approaches is that
they allow for strong guarantees: if, at any stage of refinement, our model
fails to find a solution, we can guarantee that no solution exists to the
exact problem. This allows for early exit from computation in cases where
equilibrium cannot exist. It is, to the best of our knowledge, the first time
that a model has been proposed that can handle three-dimensional frictional
constraints that include the MDP, up to arbitrary accuracy (and thus
approaching the solution to the exact problem) and in a computationally
efficient fashion.

Depending on the choice of variables and optimization objective, our
model can be used for a wide range of queries. In this paper, we
illustrate its applicability to quasi-static grasp stability analysis
by answering multiple queries on a number of example grasps. The
queries we show here include: Given applied joint torques, will the
grasp be stable in the presence of a specified external disturbance,
assuming passive resistance effects? Alternatively, given applied
joint torques, what is the largest disturbance that can be passively
resisted in a given direction? Finally, given a disturbance, what are
the optimal joint torques that a grasp can apply for stability? We
believe these are all useful tools in the context of grasp analysis,
and plan to expand the use of this model to other types of problems in
the future.

The specific queries outlined above may be of interest to roboticists only,
but an algorithm that can answer them would have applications in many other
fields faced with similar issues. In classical structural engineering, the
typical approach to solving this type of problem is to consider the
constitutive relations governing the deformation of the bodies involved. For
simple structures, this allows for an analytical computation of loads and
deformations in the system. More complex structures require approximation and
computationally intensive methods such as Finite Element Analysis. Contacts
exhibiting relative motion (i.e. sliding) further complicate these problems if
Coulomb friction is involved, as the constitutive equations determining
frictional forces at sliding contacts are non-convex.


